Unstable Motivic Homotopy Theory

We give an introduction to unstable motivic homotopy theory of Morel and Voevodsky, and survey some results.

==> figure_header.tex <==
\usepackage{tikz, xcolor}
\usetikzlibrary{calc,arrows.meta,quotes}

\pagestyle{plain}

%\def\A{\mathbf A}
%\def\P{\mathbf P}
\def\Bl{\operatorname{Bl}}

\makeatletter

\tikzset{
  myxyz/.style={x={(1cm,0cm)}, y={(-.2cm,-.8cm)}, z={(0cm,1cm)}},
  resetxy/.style={x={(1cm,0cm)}, y={(0cm,1cm)}},
}

% Apply coordinate transformation so that (1cm,0cm) is mapped to
% (xyz cs:x=1,y=0,z=#1) and (0cm,1cm) is mapped to (xyz cs:x=0,y=1,z=#1)
\newcommand\transformxy[1][0]{%
    \pgfpointxyz100%
    \pgfmathsetmacro\xx{\pgf@x/1cm}\pgfmathsetmacro\xy{\pgf@y/1cm}%
    \pgfpointxyz010%
    \pgfmathsetmacro\yx{\pgf@x/1cm}\pgfmathsetmacro\yy{\pgf@y/1cm}%
    \pgftransformcm\xx\xy\yx\yy{\pgfpointxyz00{#1}}%
  }

\tikzset{
    transformxy only/.code={\transformxy[#1]},
    transformxy only/.default=0,
    transformxy/.style={transformxy only=#1, resetxy},
    transformxy/.default=0,
}


\tikzstyle{point} = [circle, fill=black, inner sep=0pt,
                     minimum size=2mm, anchor=center]
%\def\point#1;{\@ifnextchar<{\point@overlay}{\point@nooverlay}#1;}
%\def\point@overlay<#1>#2;{\point@{#2}{<#1>}}
%\def\point@nooverlay#1;{\point@{#1}{}}
\def\point#1;{\node[point]#1{};}

\makeatother

